Observing Dialogue in Therapy: Categorizing and Forecasting Behavioral Codes

Automatically analyzing dialogue can help understand and guide behavior in domains such as counseling, where interactions are largely mediated by conversation. In this paper, we study modeling behavioral codes used to asses a psychotherapy treatment style called Motivational Interviewing (MI), which is effective for addressing substance abuse and related problems. Specifically, we address the problem of providing real-time guidance to therapists with a dialogue observer that (1) categorizes therapist and client MI behavioral codes and, (2) forecasts codes for upcoming utterances to help guide the conversation and potentially alert the therapist. For both tasks, we define neural network models that build upon recent successes in dialogue modeling. Our experiments demonstrate that our models can outperform several baselines for both tasks. We also report the results of a careful analysis that reveals the impact of the various network design tradeoffs for modeling therapy dialogue.

==> focal_loss_devices.tex <==
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> mtl_devices.tex <==
\subsection{Multiple Task Learning}
\label{ssec:mtl}

In this section, we studied whether the 4 settings in our tasks can benifit from each other.
To study the relation between annotating tasks ans forecasting task, we jointly learning the annotating tasks and forecasting task for the same speaker role as the C\_T and T\_JOINT.  To study, the relation between the client tasks and therapist task, we propose the alternative setting, our model alternative optimize for different tasks. Hence, we propose CT\_ANNO  and CT\_FORE for alternative learning for annotating tasks and forecasting task. Finally, we also proposed CT\_ALL for both alternative and jointly together, which learn our 4 settings all in one. We summerize our multple task learning settings in Table \ref{tbl:mtl}. Their experiment results are shown in Table \ref{tbl:mtl_result}

\begin{table}[tp]
\setlength{\tabcolsep}{3pt}
\begin{center}
\begin{tabular}{l|cc|cc}
\toprule
\multirow{2}{*}{ Method } & \multicolumn{2}{c|}{ Client } & \multicolumn{2}{c}{ Therapist } \\\cmidrule(lr){2-3}  \cmidrule(lr){4-5}
                          & Annotate                      & Forecast & Annotate & Forecast  \\ \midrule \midrule
C\_JOINT                  & Y                             & Y        &          &           \\
T\_JOINT                  &                               &          & Y        & Y         \\\midrule
CT\_ANNO                  & Y                             &          & Y        &           \\
CT\_FORE                  &                               & Y         &         & Y         \\ \midrule
CT\_ALL                   & Y                             & Y        & Y        & Y         \\ \midrule
\bottomrule
\end{tabular}
\end{center}
\caption{\label{tbl:mtl} Summary of Multiple Task Learning on our paper}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> pred_training.tex <==

\subsection{Predicting and Training}
\label{ssec:inference_and_training}

\Paragraph{Predicting} From up to the bottom, every component will
produce some of useful representation for inferences in our tasks.
The dialogue encoding vector $\bm{H}_{n}$, as the final of the
unidirectional GRU, it is also the contextual utterance encoding
$\bm{h}_{u_{n}}$ of $u_{n}$. Hence $H_{n}$ can be directly used as a
representaion of $u_{n}$ for classification in annotating tasks, also
can be used as a represention of whole dialogue for forecasting
task. Hence in HGRU setting, we always use $\bm{H}_{n}$ as the base
option as input for inference.

However, for CON skeleton, the final state $C_{n}$ doest not exactly
represent the segement $u_{n}$ in the whole concatnated
dalogue. Hence, we concatenate the hidden state of the start
position~(0) and end position~(T) of $u_{n}$ into
$\bm{v}^{seg}_{n}=[h_{u^{0}_{n}};h_{u^{T}_{n}}]$, which is contextual
utterance encoding in CON mode.

Beside the above $\bm{H}_{n}$ and $\bm{C}_{n}$ contextual utterance
encoding in dialogue level, our components also produced the original
utterance encoding $\bm{v}_{n}$ from utterance encoder.  Whats'more,
in \textbf{CON} mode, we can use history-aware utterance encoding $\bm{v}^{wordatt}_{n}$
While in HGRU, it produced a self-attentive utterance encoding. We
denote it as $\bm{v}^{selfatt}_{n}$.

We summarize the option input encodings for inference in Table \ref{tbl:inference}. There are two ways to scoring withthese inputs, one is to score the concatenated those vectors together, denoted as $\text{concat}(A, B)=\text{MLP}([A;B)$; The other one is scoring each of them first and then add the scores up as the final scores, such as $\text{add}(A,B)=\text{MLP}(A)+\text{MLP}(B)$.


\begin{table}[t]
\begin{center}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lcc}
\toprule
Skeleton & Annotating                                                & Forecasting  \\ \hline \hline
CON      & $\bm{v}^{seg}_{n}$,$\bm{v}^{{wordatt}_{n}}$, $\bm{v}_{n}$ & $\bm{C}_{n}$ \\ \hline
HGRU     & $\bm{H}_{n}$,$\bm{v}^{selfatt}_{n}$,$\bm{v}_{n}$          & $\bm{H}_{n}$ \\ \bottomrule
\end{tabular}
\end{center}
\caption{\label{tbl:inference_options} Input options for annotating and forecasting tasks based on CON and HGRU skeletons.}

\end{table}

% \vs{What is $t$ here? Do we have one $\alpha$ per label or example?. What
% about $\gamma$?}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> relatedwork.tex <==
\section{Related Work}

\paragraph{MISC Code Prediction} MEMM and CRF with handcrafted
features are firstly proposed by \citet{can2012case, can2015dialog}
for MISC code prediction task . Then \citet{tanana2015recursive}
improved the model by incorporating richer dependency relation
features, which even outperformed a proposed recursive neural network
baseline model. Recently, \cite{xiao2016behavioral} propose to use GRU
with domain-specific word embedding, and weighted cross-entropy loss
to resolve the label imbalance problem. In this paper, we study the
solutions draw from recent work in dialogue representation, memory
attention, and imbalanced classification. Besides that, another
improvement exists, such as topic models based domain
adaptio~\cite{atkins2014scaling, huang2018modeling}, and prosodic
features \cite{weber2002using} has been proposed to improve the
prediction tasks.

\paragraph{Dialogue Representation and Hierarchical Encoder }
End-to-End neural networks and attention mechanism has been widely
used in many natural language tasks, such as text classification,
question answering, dialogue system and so on.  RNN, CNN, and
Transformer has been quite effective for modeling sequence of
words~\cite{ kim14cnn,zhang2015character}. Combinations of them have
also been used to model the hierarchical structure of document, and
dialogue context. They first use CNN or LSTM to get a sentence vector,
and then a BiGRU to compose a sentence vectors to get a document
vector \cite{tang2015document, li2015hierarchical,
  yang2016hierarchical,sordoni2015hierarchical, serban2016building,
  serban2017multiresolution}. In our paper, we use hierarchical GRU as
skeletons. Other hierarhical combination may also help, we leave it
for future studies.

\paragraph{Attention Mechanism}
Attention mechanism was first proposed by \citet{bahdanau2014neural}
in machine translation, then various of extensions has been invented
and widely used in other tasks, especially for question answering and
dialogue
system\cite{matchlstm,bidaf,sukhbaatar15mnet,fei17gmnet,P18-1157}.
Attention on sentence-level representation also helps in many recent
works such as abstractive summarization~\cite{P18-1013}, dialogue
state tracking~\cite{zhou2018multi,zhou2016multi}, document
classification~\cite{yang2016hierarchical}.

Previous work on hierarchical attention\cite{yang2016hierarchical}
tries always to use both word-level and sentence -level attention in a
model, In this paper, we argue that, for different tasks, we need
different levels attentions. Always adding two-level attention may be
not necessary.  Recently, multi-heads multi-hops attention used in
Transformer \cite{NIPS2017_7181} became a more attractive attention
mechanism. All above advances in NLP inspired us to do systematic
analysis on whether or how they impact on our tasks.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

